Detecting and Mitigating System-Level Anomalies of Vision-Based Controllers

Autonomous systems, such as self-driving cars and drones, have made significant strides in recent years by leveraging visual inputs and machine learning for decision-making and control. Despite their impressive performance, these vision-based controllers can make erroneous predictions when faced with novel or out-of-distribution inputs. Such errors can cascade to catastrophic system failures and compromise system safety. In this work, we introduce a run-time anomaly monitor to detect and mitigate such closed-loop, system-level failures. Specifically, we leverage a reachability-based framework to stress-test the vision-based controller offline and mine its system-level failures. This data is then used to train a classifier that is leveraged online to flag inputs that might cause system breakdowns. The anomaly detector highlights issues that transcend individual modules and pertain to the safety of the overall system. We also design a fallback controller that robustly handles these detected anomalies to preserve system safety. We validate the proposed approach on an autonomous aircraft taxiing system that uses a vision-based controller for taxiing. Our results show the efficacy of the proposed approach in identifying and handling system-level anomalies, outperforming methods such as prediction error-based detection, and ensembling, thereby enhancing the overall safety and robustness of autonomous systems.

==> intro.tex <==
% The utilization of robots within safety-critical systems has experienced a steady increase over time. 
% 
With the advances in deep learning and computer vision, modern autonomous and robotic systems have reached a level of competence that, in some instances, exceeds human capabilities \cite{kaufmann2023champion}. 
Nevertheless, in the context of safety-critical systems, ensuring that these algorithms undergo rigorous verification for potential failures before they are deployed in real-world scenarios is imperative. 
Such failures may manifest due to the incapacity of machine learning algorithms to comprehend the underlying data patterns (referred to as functional uncertainty) or due to inherent variations in the data itself, which presents a formidable challenge to address (known as distribution shifts). The process of identifying data instances that could lead to undesirable system behavior is commonly referred to as anomaly detection. 

Anomaly detectors (AD) are essential for robotic systems, especially with a learning framework, to prevent unwanted behavior \cite{sinha2022system}. However, determining if the input is anomalous is not a trivial problem \cite{gupta2018open}. As a first step, knowing what constitutes an anomaly requires expert domain knowledge and exhaustive searches for counterexamples. Studies \cite{sun2021complementing} have attempted to introduce noise in the ground truth image data in an effort to force a shift in the underlying distribution to artificially create anomalous data. Yet such artificial perturbations in high dimensional data may completely alter the base distribution to produce unrealistic images.

Due to the difficulty of understanding domain-specific anomalies, another approach is to focus on functional uncertainty - if a system deviates too much from a predetermined nominal behavior under the given inputs, these inputs are anomalous. The extent to which the system is allowed to vary is often determined heuristically or empirically. These methods have shown promise in applications like industrial robotic arms \cite{narayanan2018learning} and agricultural robots \cite{ji2022proactive} where the environment does not change too much from training to test time, and hence the formulation of a predefined nominal trajectory is not infeasible. However, obtaining such a nominal behavior is a non-trivial challenge if the robot encounters a novel scenario or situation such as sim-to-real transfer. For such cases, researchers have seen appreciable success using a learned classifier \cite{sun2021complementing} or concepts like normalizing flows or GANs \cite{mantegazza2022outlier}. Nevertheless, a common requirement across all these methods remains a significant domain knowledge to formulate a nominal system behavior or generate logical anomaly scenarios. 

Due to the requirement of runtime or deployment verification, considerable efforts have been directed toward developing frameworks capable of detecting failures at both the system and module levels \cite{rahman2021run}. These include rigorous verification of the input-output relation of neural networks \cite{tjeng2017evaluating,katz2017reluplex}, which provide certification of output correctness through the generation of counterexamples. Pipelines such as ALERT \cite{zhang2014predicting} produce a confidence score enabling the identification of spurious outputs produced by computer vision algorithms. 
% Armed with such bounds or confidence scores, one can make informed decisions regarding the acceptance or rejection of the algorithmic predictions.

Nonetheless, the guarantees provided by the underlying submodules are often not representative of the overall system's performance. Seemingly minor errors in the individual modules can cascade into catastrophic effects at a system level. Hence, a system-level view of such problems is often encouraged and is the main motivation behind this work.

 
There has been significant focus on the detection of closed-loop system failures, using techniques like system verification\cite{huang2019reachnn, xiang2018output, julian2019guaranteeing,lin2020reachflow}, GANs \cite{katz2021verification}, monitoring invariants \cite{jiang2017inferring}, or geometric sensor mappings \cite{santa2022nnlander}. However, these methods are limited in application by the low dimensionality inherent to the underlying systems being verified or by abstracting the intricacies associated with high-dimension systems. Innovations in modern photorealistic simulators have presented an opportunity for employing forward simulations \cite{fremont2020formal, dreossi2017systematic} or falsification \cite{ghosh2021counterexample} as viable means for closed-loop falsifications of such systems. However, it is essential to acknowledge that these methods encounter a significant hurdle in time complexity, rendering them computationally infeasible.

In a study conducted by Chakraborty et al. \cite{chakraborty2023discovering}, an innovative approach is presented, wherein the challenge of identifying closed-loop failures within visual navigation pipelines is reformulated as a Hamilton-Jacobi (HJ) reachability problem. This approach employed a grid-based reachability solver to approximate a backward-reachable tube (BRT) by utilizing samples obtained from a photorealistic simulator. The method effectively identified that visual inputs falling inside the confines of the BRT resulted in system failure. This method addressed the challenge posed by the high dimensionality inherent in the system and demonstrated satisfactory performance for systems characterized by up to five dimensions.

Taking inspiration from such work, in this paper, we propose an anomaly detector (AD) that can detect the failure modes of systems that use visual inputs from their environment. Our AD leverages insights garnered from the revealed failure modes to classify whether a previously unseen input image has the potential to trigger a system failure. To reduce the dependence on expert intervention, we propose an automatic labeling scheme to create an anomaly dataset using the BRT obtained from the reachability analysis of the closed-loop system. In addition to not requiring any heuristic or specific domain knowledge, the BRT-based labels have the added advantage of encoding the closed-loop failures of the system. 

However, knowing if an input signal is anomalous is insufficient to mitigate the system's failures. Failsafe mechanisms \cite{saxena2017learning,lin2020reachflow} are required to ensure the system's safety with minimum external intervention. We employ a simple fallback controller that can trade the system's performance to assure system safety whenever the anomaly detector determines the system is at risk of entering the failure zone. We demonstrate the joint properties of our anomaly detector and fallback controller in two distinct cases: (i) autonomous aircraft taxiing and (ii) indoor navigation for a wheeled robot. In the first case, we use a velocity controller-based fallback controller that slows down the system if the anomaly detector is triggered, while in the second case, we use a SLAM-based pipeline that can plan on a previously known map once the system behavior shows anomalous patterns.

In summary, for closed-loop visual-controller-based robotic systems, we propose:
\begin{itemize}
    \item An HJ Reachability-inspired method for generating an anomaly detection dataset.
    \item A learned anomaly detector that can discern if an input image can lead to closed-loop system failure.
    \item A fallback controller that can maintain the safe operation of the system depending on the predictions from the anomaly detector. 
\end{itemize}

We compare our method against commonly used techniques such as ensemble uncertainty and prediction error-based anomaly detectors to show the performance of our method over general anomaly detection algorithms.

% In other words, our anomaly detector can learn and predict the failures of closed-loop robot systems that utilize visual controllers.

% For example, an error involving the misclassification of a few pixels within a semantic segmentation algorithm may be considered minor within the context of module-based verification. However, this seemingly minor error can have cascading consequences, potentially causing an autonomous vehicle to veer off its lane on a high-speed freeway.



% Robotic systems often consist of multiple interconnected submodules functioning in a closed-loop fashion to achieve specific objectives. Autonomous systems like self-driving cars \cite{majumdar2023robotics} serve as quintessential examples of such systems, comprising submodules such as perception stacks, planners, and controllers. 







% Given the BRT and image samples from the systems's observable state space, if a particular sampled image is a part of the system's BRT then the image is labeled as an anomaly. 



% To tackle this search for a general pipeline, we propose a deep neural network inspired by the EfficientNet \cite{tan2019efficientnet} as a learned classifier-based AD. Supervised training via the labels derived from the system's BRT, allows our AD to detect anomalies that lead to closed-loop failures. Moreover, it was seen to learn some cases of semantic failure which needed to be manually determined before \cite{chakraborty2023discovering}.



==> performance_table.tex <==
\begin{table}[htbp]
\caption{Performance of Anomaly Detector on Different Airports at Various Times of Day and Cloud Conditions} 
% \setlength{\tabcolsep}{4pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{@{}ccccc@{}}
% \begin{tabular*}{\linewidth}{@{}ccccc@{}}
\hline
\rule{0pt}{1\normalbaselineskip}
\textbf{Airport ID} & \textbf{Time} & \textbf{Cloud Condition} & \textbf{Recall} (\%) & \textbf{Accuracy} (\%) \\[1mm]
\hline
\rule{0pt}{1\normalbaselineskip}
KMWH                & 5 PM                 & Clear                    & 91.50                & 95.89                  \\
KMWH                & 5 PM                 & Overcast                 & 92.22                & 97.02                  \\[1mm]
\hline
\rule{0pt}{1\normalbaselineskip}
KATL                & 5 PM                 & Clear                    & 97.44                & 98.19                  \\
KATL                & 5 PM                 & Overcast                 & 95.89                & 97.97                  \\[1mm]
\hline
\rule{0pt}{1\normalbaselineskip}
PAEI                & 5 PM                 & Clear                    & 93.24                & 97.71                  \\
PAEI                & 5 PM                 & Overcast                 & 93.71                & 97.99                  \\[1mm]
\hline
\rule{0pt}{1\normalbaselineskip}
KEWR                & 9 AM                 & Clear                    & 90.60                & 95.75                  \\
KEWR                & 9 AM                 & Overcast                 & 92.61                & 96.75                  \\
KEWR                & 5 PM                 & Clear                    & 96.31                & 96.29                  \\
KEWR                & 5 PM                 & Overcast                 & 94.20                & 96.72                  \\
KEWR                & 9 PM                 & Clear                    & 87.42                & 94.72                  \\
KEWR                & 9 PM                 & Overcast                 & 90.49                & 95.56                  \\[1mm]
\hline
\rule{0pt}{1\normalbaselineskip}
KSFO                & 9 AM                 & Clear                    & 90.27                & 91.51                  \\
KSFO                & 9 AM                 & Overcast                 & 90.61                & 89.81                  \\
KSFO                & 5 PM                 & Clear                    & 90.34                & 89.72                  \\
KSFO                & 5 PM                 & Overcast                 & 90.56                & 90.62                  \\
KSFO                & 9 PM                 & Clear                    & 85.32                & 86.44                  \\
KSFO                & 9 PM                 & Overcast                 & 86.91                & 87.32                  \\[1mm]
\hline
\label{table:performance_table}
\end{tabular}}
\end{table}

==> related.tex <==
Related works go here

==> table1.tex <==
\begin{table}[htbp]
\centering
\caption{Performance of Anomaly Detector on Different Airports at Various Times of Day and Cloud Conditions}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccc}
\hline
\rule{0pt}{1\normalbaselineskip}
\multirow{2}{*}{\textbf{Airport ID}} & \multirow{2}{*}{\textbf{Time of Day}} & \multicolumn{2}{c}{\textbf{Recall (\%)}} & \multicolumn{2}{c}{\textbf{Accuracy (\%)}} \\
                                     &                                       & (C)                 & (O)                & (C)                  & (O)                 \\[1mm]
\hline
\rule{0pt}{1\normalbaselineskip}
KMWH                                 & 5 PM                                  & 91.50               & 92.22              & 95.89                & 97.02               \\
KATL                                 & 5 PM                                  & 97.44               & 95.89              & 98.19                & 97.97               \\
PAEI                                 & 5 PM                                  & 93.24               & 93.71              & 97.71                & 97.99               \\
KEWR                                 & 9 AM                                  & 90.60               & 92.61              & 95.75                & 96.75               \\
KEWR                                 & 5 PM                                  & 96.31               & 94.20              & 96.29                & 96.72               \\
KEWR                                 & 9 PM                                  & 87.42               & 90.49              & 94.72                & 95.56               \\
KSFO                                 & 9 AM                                  & 90.27               & 90.61              & 91.51                & 89.81               \\
KSFO                                 & 5 PM                                  & 90.34               & 90.56              & 89.72                & 90.62               \\
KSFO                                 & 9 PM                                  & 85.32               & 86.91              & 86.44                & 87.32              \\[1mm]
\hline
\label{table:table1}
\end{tabular}%
}
\end{table}

==> waypointnav.tex <==
\subsection{Autonomous Visual Navigation in Indoor Environments}
Our second case study analyzes the autonomous navigation of a wheeled robot in an indoor environment \cite{bansal2020combining}. The robot is modeled as a 5-dimensional nonlinear system with dynamics:
\vspace{-0.6em}
\begin{align*}
\label{eqn:dyn_lbwpn}
        \dot p_x = v cos(\theta),~\dot p_y = v sin(\theta),~\dot \theta = \omega,~\dot v = a,~\dot \omega = \alpha
        \vspace{-2em}
\end{align*}
% 
where $p_x$ and $p_y$ denote the xy-position of the robot, $\theta$ is the robot heading, and $v \text{ and } \omega$ are its linear and angular speeds. The robot is assumed to have access to perfect state estimates. The control, denoted as $\ctrl \coloneqq (a,\ \alpha)$, comprises linear acceleration (a) and angular acceleration ($\alpha$). The navigation pipeline is a convolutional neural network (CNN) denoted as $C$, which takes a $224x224x3$ RGB image $\image$ from an onboard camera, instantaneous linear and angular speeds of the robot ($v$ and $\omega$), and a goal position ($g$) to predict an intermediate waypoint for the robot's movement. Additionally, a model-based spline planner $P$ uses this predicted waypoint to generate a smooth control profile for the robot. Therefore, the policy $\hat \policy$ can be expressed as $\hat \policy := P \circ C \circ \sensor(\state, g)$. Given a robot state, use the Stanford Building Parser Dataset (SBPD) \cite{SBPD} renderer generate photo-realistic images ($\image = \sensor(\state)$) of indoor scenes taken by a virtual monocular RGB camera $\sensor$, mounted on the robot. Note that the obstacles are unknown to the robot, and it must navigate only using first-person RGB images.

We aim to find the AD $\classy$ for ($\hat \policy$) to identify anomalous images $\image \in \ibrt$ that lead to the system failure. Here, ``failure" is defined as the robot's incapability to reach its intended goal within a time span of 50 seconds. Failures can occur for various reasons, such as collisions with obstacles or the control process taking an excessively long time to reach the goal, resulting in a timeout situation.



\noindent \textbf{\textit{Generation of an Anomaly Dataset for Autonomous Navigation of Wheeled Robot.}}
The procedure for the dataset generation is identical to the TaxiNet case study with two major differences: firstly, we compute the Backward Reach-Avoid Tube (BRAT, instead of the BRT), and secondly, images from any state not contained in the BRAT are now labeled as anomalies (in contrast to the TaxiNet case where the images in the BRT are labeled as anomalies). The BRAT is the set of states from which the robot reaches its goal without colliding with obstacles. A representative BRAT for 50 seconds and some training images are shown in Fig. XYX \kccom{will add a brat and some images}. BRAT can be computed by similarly solving the HJB-VI as BRT, with an additional constraint that the robot trajectory terminates once it reaches the goal. The complement of the BRAT thus represents the unsafe states for the robot under $\hat \policy$.


We used 4 areas (numbered 1 through 4) with distinct features from the SBPD dataset. We chose 3 patches of 10 sq. meters each from Area 1 as our training dataset and used random rollouts from Areas 4,5,6 \kccom{check with this} in our test set. \kccom{how many rollouts} Note that the grid-based level set method for BRAT computation suffers from the curse of dimensionality. Hence, while dealing with this 5D system, we were constrained to choose small patches ($10\,m^2$) for our training scenario. Future work will explore the computation using methods like DeepReach that scale well with grid resolution and dimensions. 

\noindent \textbf{\textit{Anomaly Detector.}} We keep the structure of the anomaly detector the same as our previous case. This decision was driven by the choice to introduce a comprehensive framework in which the focus lies on the quality of the training data rather than the neural network architecture while dealing with completely different systems. We added standard data augmentation methods such as randomly distorting brightness and contrast and adding blur\kccom{Aryaman: please list what you added.} to prevent overfitting even with a relatively small dataset. 
\noindent \textbf{\textit{Evaluation.}} We summarise the AD's performance on the unseen areas comprising our training set in Table. \kccom{Aryaman please add table}. The AD again displays a high recall, showing the conservative nature of our network while the overall accuracy of XY\% demonstrates that the AD was able to learn the underlying features of anomalous images for the indoor navigation task. Looking into some representative images that were classified as anomalous, we listed some interesting behaviors:
\begin{enumerate}
    \item Interesting failure 1......
\end{enumerate}
\noindent \textbf{\textit{Fallback controller.}} For the fallback controller, we employ a Model Predictive Control (MPC) pipeline that has access to the occupancy map of the area and can determine waypoints via optimal control, which we call the expert controller. If any input to the system is deemed anomalous by our AD, we use the prediction from our expert as the final input to the system; otherwise, we use the vision-based controller predictions. One may choose any other fallback controller instead of the MPC to handle anomalous vision inputs. Some commonly used choices are visual-SLAM or employing richer sensors like LiDARs, which may be expensive to process but are more accurate. Our fallback controller was able to retrieve the system from states that were deemed as failures by the AD. These include... \kccom{demonstate the fallback controller}

{\textbf{\textit{Baselines.}}}
\subsubsection{Prediction Error-based Labels} Similar to the TaxiNet case, we implemented an error-prediction labeling system (depicted in Figure \ref{fig:waypointnav_error_baseline}) across three distinct thresholds. For a particular state, the error is calculated by the Euclidean distance of the predicted waypoint to the expert waypoint. If the error is above a certain threshold, then we classify that state as a failure state (magenta region in the figure) and the corresponding image as an anomaly. 
%
\begin{figure}[h]
    \centering
    \vspace{-0.75em}
         \includegraphics[width=0.85\columnwidth]{images/waypointnav_error_labels.png}
        \caption{\small{Error based labels for different thresholds \textbf{(a)} 0.15, \textbf{(c)} 0.25, \textbf{(c)} 0.40,  for a specific start heading (indicated by the arrow in the top left of each plot) and velocities shown on a top-view occupancy map with the obstacles shown in grey. The magenta region highlights areas that the error-based method predicts as potential failures. The teal region shows the BRAT. The green circle, marked with a black star at the origin, represents the goal location.  Lower threshold values result in false negatives, while higher values of threshold result in false positives. }}
         \vspace{-0.75em}
         \label{fig:waypointnav_error_baseline}
\end{figure}
%
Ideally, the magenta region should cover all the white areas since they depict areas where the robot fails to reach the goal. When employing a small threshold (0.15), these error-based labels struggle to pinpoint failure areas effectively; consequently, an AD trained on such labels will be optimistic, classifying most input images as safe even when anomalous. This propensity for false negatives results in a higher incidence of system failures.
On increasing the threshold ($0.25$, $0.40$), the labels become more conservative. Now, even safe images are erroneously tagged as anomalies, albeit some failure regions remain unlabeled as anomalous, showing the issues pertinent to component-level analysis. Our BRT-based AD is able to strike a balance between accuracy and recall, ensuring the development of a reliable fallback controller while minimizing excessive conservatism.

\subsubsection{Ensemble Predictions} In this approach, we train an ensemble of 5 CNNs with random initialization of the weights to achieve an average of 70\% accuracy over a testing dataset. For any input image, if the variance of the predictions over all the ensemble members exceeded a certain threshold, we classify such an input as anomalous. Fig. \ref{fig:wpnav_ensemble} shows the ensemble labels over the BRAT-based labels on the occupancy grid.
% 
\begin{wrapfigure}{r}{0.40\columnwidth}
          \centering
          \vspace{-1.5em}
         \includegraphics[width=0.35\columnwidth]{images/waypointnav_ensemble_labels.png}
         \vspace{-0.5em}
         \caption{\small{Labels generated using ensembling denoting Failure (magenta).}}
         \vspace{-1.5em}
         \label{fig:wpnav_ensemble}
\end{wrapfigure}
% 
Again, this method was deemed unreliable since it was seen that all the members of the ensemble confidently made incorrect predictions for most of the states, classifying them as safe states. We observed a pattern where the labels looked as if the ensemble was failing on states starting with specific x-axis positions. Hence, irrespective of the other parameters, the ensemble performs incorrectly for those states.



